On Misspecification in Prediction Problems and Robustness via Improper Learning

We study probabilistic prediction games when the underlying model is misspecified, investigating the consequences of predicting using an incorrect parametric model. We show that for a broad class of loss functions and parametric families of distributions, the regret of playing a "proper" predictor -- one from the putative model class -- relative to the best predictor in the same model class has lower bound scaling at least as $\sqrt{\gamma n}$, where $\gamma$ is a measure of the model misspecification to the true distribution in terms of total variation distance. In contrast, using an aggregation-based (improper) learner, one can obtain regret $d \log n$ for any underlying generating distribution, where $d$ is the dimension of the parameter; we exhibit instances in which this is unimprovable even over the family of all learners that may play distributions in the convex hull of the parametric family. These results suggest that simple strategies for aggregating multiple learners together should be more robust, and several experiments conform to this hypothesis.

==> sections/convexhull.tex <==
A substantial amount of research in the area of probabilistic forecasting has provided motivating applications and considered the problem of how to optimally return distributions from $\conv \param$, but has also left much unanswered; see \citep{GrangerRa84, GenestZi86, Clemen89, Jacobs95, HsuCh96, ClemenWi99, HallMi07} for a general review. We hope that this paper, in showing the minimax risk stability achieved by working in the convex hull, provides further motivation to continue research in this direction. 
\paragraph{An instance where returning a distribution from the convex hull achieves arbitrarily improved risk:} In what follows we consider an example in which the class $\param$ has no predictive power while the class $\conv \param$ achieves risk converging to $0$. Given $n$, consider the distribution over pairs $(X,Y)$:
\begin{equation*}
P_{n}(X,Y) = \begin{cases}
\frac{1}{1+n}, \tr{ if } (X,Y) = (-n,1), \\
\frac{n}{1+n}, \tr{ if } (X,Y) = (1,1).
\end{cases}
\end{equation*}
We are interested in the difference in risk, as measured by log-loss, between returning a distribution from the family $\param$ where $P_{\theta}(y \lvert x) = (1+\exp(-y\theta^{T}x))^{-1}$ and returning a distribution from $\conv \param$. We will show that the best risk achievable from $\param$ is the same as the risk achieved by trivially returning the uniform distribution over the data. On the other hand, we will show that simply returning a two-point mixture from $\conv \param$ achieves risk converging to $0$ as $n \to \infty$. To this end, one can first check that $\theta = 0$ achieves the optimal risk for each $P_{n}$, 
\begin{align*}
& \nabla_{\theta} \E_{P_{n}}[-\log( P_{\theta}(Y \lvert X))]  \big \lvert_{\theta = 0} \\
=& \nabla_{\theta} \bigg[ \frac{1}{1+n} \log(1+\exp(n\theta))  \\
& \qquad + \frac{n}{1+n} \log(1 + \exp(-\theta)) \bigg] \big \lvert_{\theta = 0} =0.
\end{align*}
Thus the best $P_{\theta^*}$ can do no better than trivially returning a uniform distribution over the data. On the other hand, consider the two-point mixture $P_{\tr{mix},n} = \frac{1}{n}P_{0} + (1-\frac{1}{n})P_{n}$. Then we find that
\begin{align*}
& \lim \limits_{n \to \infty} \E_{P_{n}}[-\log(P_{\tr{mix},n}(Y \lvert X))] \\
=  & \lim \limits_{n \to \infty} \frac{-1}{1+n} \log \bigg( \frac{1}{2n} + \frac{1-\frac{1}{n}}{1+e^{n^{2}}} \bigg) \\
& \qquad - \frac{n}{n+1} \log \bigg( \frac{1}{2n} + \frac{1 - \frac{1}{n}}{1 + e^{-n}} \bigg) = 0,
\end{align*}
that is the risk induced by $P_{n}$ converges to $0$ as $n \to \infty$. This motivates the general question: how superior is the risk performance of simply the best two-point mixture of parameterized distributions? Do there exist any efficient algorithms to compute it? To our knowledge, this question remains unanswered.
